Adaptive Convolutions

When smoothing a function $f$ via convolution with some kernel, it is often desirable to adapt the amount of smoothing locally to the variation of $f$. For this purpose, the constant smoothing coefficient of regular convolutions needs to be replaced by an adaptation function $\mu$. This function is matrix-valued which allows for different degrees of smoothing in different directions. The aim of this paper is twofold. The first is to provide a theoretical framework for such adaptive convolutions. The second purpose is to derive a formula for the automatic choice of the adaptation function $\mu = \mu_f$ in dependence of the function $f$ to be smoothed. This requires the notion of the \emph{local variation} of $f$, the quantification of which relies on certain phase space transformations of $f$. The derivation is guided by meaningful axioms which, among other things, guarantee invariance of adaptive convolutions under shifting and scaling of $f$.

==> sections/ChoiceAdaptationFunctionAlt.tex <==
\section{Choice of a Proper Adaptation Function $\mu$}
\label{section:ConvolutionAdaptationFunction}

In the example from Section \ref{section:convolutionMotivation}, the adaptation
function $\mu$ was chosen \emph{manually} to smooth the function $f:\R^d\to\R$
in a reasonable way, when taking the $\mu$-adapted convolution with the density
$g$.
Let us now discuss how this choice can be performed \emph{automatically} in
dependence of the function $f$ that we want to smooth.

Finding a good dependence for the adaptation function $\mu = \mu_f$ on the
function $f$ is a difficult task and will only be partially answered here.
We will justify the choice
\[
\mu_f(x) = \sqrt{\frac{(f^2)\ast(\nabla f\cdot\nabla f^T - f D^2
f)}{4\, (f^2)\ast(f^2)}\, (2x)},
\]
but neither prove uniqueness, nor any kind of optimality.
Also, we will restrict ourselves to radially symmetric smoothing kernels $g$,
i.e. $g(x) = \gamma(\|x\|^2)$ for some function $\gamma\colon \R\to\R$.

\begin{remark}
The square root of a symmetric and positive definite matrix $M$ will denote
the upper triangular factor in its Cholesky decomposition:
\[
\sqrt{M}:= L^T,\qquad\text{where } M = LL^T\text{ and $L$ is lower
triangular.}
\]
\end{remark}

Let us first gather some criteria, which we would like our adaptation function
$\mu_f$ to fulfill (see also the motivation in Section
\ref{section:convolutionMotivation}):
\begin{condition}[Adaptation Conditions]
\label{cond:adaptation}
From now on we will say that the mapping $f\mapsto \mu_f$ fulfills the
\emph{Adaptation Conditions}, if it has the following properties:
\begin{enumerate}[(i)]
  \item Invariance under shifting by some vector $a\in\R^d$:
  $\hspace{1.3cm}\displaystyle
  \mu_{f(\Cdot\, - a)}(x) = \mu_f(x-a)$.
  \item Invariance under multiplication by some factor $\alpha\neq 0$:
  $\hspace{0.4cm}\displaystyle \mu_{\alpha\cdot f} = \mu_f$.
  \item Scaling when $f$ is scaled by some matrix
  $A\in\gldr$:
  \[
  \mu_{f(A\cdot\, \Cdot)}^{\intercal}(x)\, \mu_{f(A\cdot\, \Cdot)}(x)
  =
  A^{\intercal}\, \mu_f(A x)^{\intercal}\, \mu_f(A x)\, A.
  \]  
%   $A\in\gldr$: $\quad\displaystyle
%   \mu_{f(A\cdot\, \Cdot)}(x) = \sqrt{A^{\intercal}\mu_f(A x)^{\intercal}\mu_f(A
%   x)A}$
  \item $\mu_f(x)$ should describe some kind of ``variation'' of
  $f$ locally around $x\in\R^d$.
\end{enumerate}
\end{condition}

These conditions are chosen in such a way that the
$\mu_f$-adapted convolution behaves nicely under shifting and scaling of $f$, as
stated in the following lemma:
\begin{lemma}
Let $\mu\colon L^1\to \gldr,\ f\mapsto \mu_f$ fulfill the Adaptation Conditions
(i)--(iii), $g\in L^p$ be radially symmetric, $a\in\R^d,\
\alpha\in\R\setminus{0}$ and $A\in\gldr$.
\\
Then for all $f\in L^1$, we have
\begin{enumerate}[(i)]
  \item $\displaystyle (f(\Cdot\, - a)\ast^p_{\mu_{f(\Cdot\, - a)}} g) (x)=
  (f\ast^p_{\mu_f}g) (x-a)$,
  \item $\displaystyle (\alpha f\ast^p_{\mu_{\alpha f}} g) (x)=
  \alpha (f\ast^p_{\mu_f}g) (x)$,
  \item $\displaystyle (f(A\cdot\Cdot)\ast^p_{\mu_{f(A\cdot\Cdot)}} g) (x)=
  (f\ast^p_{\mu_f}g) (Ax)$.
\end{enumerate}
\end{lemma}


\begin{proof}
Again, let $g(x) = \gamma(\|x\|^2)$ for some function $\gamma\colon \R\to\R$. We have:
\begin{align*}
&(f(\Cdot\, - a)\ast^p_{\mu_{f(\Cdot\, - a)}} g) (x)
=
\int f(y-a) \left|\det\left(\mu_{f}(y-a)\right)\right|
g\left(\mu_{f}(y-a)(x-y)\right)\, \mathrm dy
\\
& \hspace{1cm} =
\int f(y) \left|\det\left(\mu_{f}(y)\right)\right|
g\left(\mu_{f}(y)(x-a-y)\right)\, \mathrm dy
\\
& \hspace{1cm} =
(f\ast^p_{\mu_f}g) (x-a),
\\[0.2cm]
&(\alpha f\ast^p_{\mu_{\alpha f}} g) (x)
=
\int \alpha f(y) \left|\det\left(\mu_{f}(y)\right)\right|
g\left(\mu_{f}(y)(x-y)\right)\, \mathrm dy
=
\alpha (f\ast^p_{\mu_f}g) (x),
\\[0.2cm]
&(f(A\cdot\Cdot)\ast^p_{\mu_{f(A\cdot\Cdot)}} g) (x)
=
\int f(Ay) \left|\det\left(\mu_{f(A\cdot\Cdot)}(y)\right)\right|
g\left(\mu_{f(A\cdot\Cdot)}(y)(x-y)\right)\, \mathrm dy
\\
& \hspace{1cm} =
\int f(Ay) \left|\det\left(\mu_f(A
y)A\right)\right| \gamma\big((x-y)^{\intercal}A^{\intercal}\mu_f(A
y)^{\intercal}\mu_f(A y)A(x-y)\big)\, \mathrm dy
\\
& \hspace{1cm} =
\int f(y) \left|\det\left(\mu_f(y)\right)\right| \gamma\big((Ax-y)^{\intercal}
\mu_f(y)^{\intercal}\mu_f(y)(Ax-y)\big)\, \mathrm dy
\\
& \hspace{1cm} =
\int f(y) \left|\det\left(\mu_f(y)\right)\right| g\big( \mu_f(y)(Ax-y)\big)\,
\mathrm dy
\\
& \hspace{1cm} =
(f\ast^p_{\mu_f}g) (Ax).
\end{align*}
\end{proof}



\begin{remark}
Adaptation Condition (iii) is a necessary detour around the more appealing
condition
\[
\mu_{f(A\cdot\, \Cdot)}(x) = \mu_f(Ax)A,
\]
since the product of a triangular matrix with an invertible matrix is not
triangular in general. This is also the reason why we are only able to
treat radially symmetric smoothing kernels $g$. Roughly speaking, covariance
matrices are easier to treat than their square roots.
\end{remark}


One possible choice that fulfills the Adaptation Conditions (i)--(iii) is
\[
\mu_f = \sqrt{\frac{\nabla f\nabla f^{\intercal}}{f^2}}.
\]
However, $\nabla f\nabla f^{\intercal}$ is only positive \emph{semi}-definite
and therefore $\mu_f\in\gldr$ could be violated. Also, it
is unclear in how far the Adaptation Condition (iv) is fulfilled.
Obviously, this condition is not rigorous and we will discuss it now. In order
to get a grasp on it, we will make use of three transformations
explained in the following subsection.










\subsection{Phase Space Transformations}
\label{section:PhaseSpace}

In this section, we will discuss three transformations, which allow us to
comprehend the (local) variation of a function.
All three transformations can be viewed from various perspectives and we will
focus on the time-frequency point of view. In the following, $\mathcal
S(\R^d,\C)$ will denote the Schwartz space of rapidly decreasing functions.

\begin{definition}[Gaussian, Fourier transform, windowed Fourier transform,
Wigner transform]
We define
\begin{enumerate}[(i)]
  \item the \emph{Gaussian function} $G[a,\Sigma]\colon \R^d\to\R$ with mean
  $a\in\R^d$ and symmetric and positive definite covariance matrix $\Sigma\in\gldr$,   
  \item the \emph{Fourier transform} $\F: \mathcal S(\R^d,\C)\to \mathcal
  S(\R^d,\C)$,
  \item the \emph{windowed Fourier transform} $\F_{\sigma}:
  \mathcal S(\R^d,\C)\to \mathcal S(\R^d\times \R^d,\C)$ with window width
  $\sigma>0$,
  \item the \emph{Wigner transform} $W: \mathcal S(\R^d,\C)\to \mathcal
  S(\R^d\times\R^d,\R)$ by
\footnote{Usually, the Wigner transform
%$W: \mathcal S(\R^d,\C)\times S(\R^d,\C)\to \mathcal S(\R^d\times\R^d,\C)$
is defined by
$
% \displaystyle
W(f,g)(x,\xi) = (2\pi)^{-d}\int_{\R^d}\overline{f\left(x+\frac{y}{2}\right)}\,
g\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy.
$
We will only use its definition on the diagonal, $Wf := W(f,f)$, where it is
real-valued, which can be seen by applying the transformation $y\mapsto -y$ to
the integral.}
\end{enumerate}
\vspace{-0.6cm}
\begin{align}
\label{equ:generalGaussian}
G[a,\Sigma](x)
&=
(2\pi)^{-d/2}\, |\det \Sigma|^{-1/2}\,
\exp\left[-\frac{1}{2}(x-a)^{-\intercal}\Sigma^{-1} (x-a)\right],
\\
\mathcal F f (\xi)
&=
(2\pi)^{-d/2} \int_{\R^d} f(y)\, e^{-iy^\intercal\xi}\,
\mathrm dy\, ,
\\
\label{equ:windowedFourier}
\F_{\sigma} f(x,\xi)
&=
\pi^{-d/4} \int_{\R^d}f(y)\, G[0,\sigma\, \Id](x-y)\,
e^{-iy^\intercal\xi}\, \mathrm dy\, ,
\\
Wf(x,\xi)
&=
(2\pi)^{-d}\int_{\R^d}\overline{f\left(x+\frac{y}{2}\right)}\,
f\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy.
\end{align}
\end{definition}





We will restrict ourselves to presenting only few properties of these
transforms, further properties can be found in e.g. \cite{folland1989harmonic}.

\begin{proposition}[Plancherel Theorem and Fourier Inversion Formula]
\label{prop:fourierInverse}
\ \\
The Fourier transform is an isometric isomorphism with inverse
\[
\mathcal F^{-1} f(x) = (2\pi)^{-d/2} \int_{\R^d} f(\xi)\,
e^{-ix^\intercal\xi}\, \mathrm d\xi\, .
\]
\end{proposition}
\begin{proof}
See \cite{folland1989harmonic}.
\end{proof}
The Fourier inversion formula implies for $f\in\mathcal S(\R^d,\C)$
\[
(2\pi)^{-d} \int_{\R^d} \int_{\R^d} f(x)\,
e^{-ix^\intercal\xi}\, \mathrm d\xi\, \mathrm dx
\ =\ 
(2\pi)^{-d/2} \int_{\R^d} \F f(\xi)\,  e^{i0^\intercal\xi}\, \mathrm d\xi\, 
\ =\ 
\F^{-1}\F f(0)
\ =\ 
f(0). 
\]
The technique of using ``$(2\pi)^{-d}\int_{\R^d} e^{-ix^\intercal\xi}\, \mathrm
d\xi$'' as a $\delta$-distribution will be used several times in this section.


From the point of view of time-frequency analysis, the Fourier transform yields a
decomposition of the signal $f$ into its frequencies: for each frequency $\xi$,
it indicates the extent of its occurrence in $f$.
However, one is often interested in the local frequencies of $f$, meaning, which
frequencies of $f$ occur at (or close to) a specific
point in time $x$.
This can be analyzed using a windowed Fourier transform, also called Gabor transform, which does not
``see'' the values and frequencies of $f$ far from $x$. Applied to each
point in time $x$, this defines the mapping \eqref{equ:windowedFourier} on the
phase space.

\begin{figure}[H]
\centering
\begin{subfigure}[b]{0.097\textwidth}
	\centering	
	\includegraphics[width=4\textwidth,angle = 	90]{images/FBI_Wigner2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.388\textwidth}
	\centering	                
	\includegraphics[width=\textwidth]{images/FBI_Wigner3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.388\textwidth}
	\centering	                
	\includegraphics[width=\textwidth]{images/FBI_Wigner4}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.097\textwidth}
	\centering	
	\includegraphics[width=0.77\textwidth]{images/FBI_Wigner5}
\end{subfigure}

\vfill
\vspace{0.3cm}

\begin{subfigure}[b]{0.097\textwidth}
	\centering
	\phantom{\includegraphics[width=0.94\textwidth]{images/FBI_Wigner3}}	
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.388\textwidth}
	\centering
	\includegraphics[width=\textwidth]{images/FBI_Wigner1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.388\textwidth}
	\centering
	\includegraphics[width=\textwidth]{images/FBI_Wigner1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.097\textwidth}
	\centering
	\phantom{\includegraphics[width=\textwidth]{images/FBI_Wigner3}}
\end{subfigure}
\caption{Visualisation of how different frequencies of a function $f$ are
represented by the Fourier transform $\F f$, the windowed Fourier transform
$\F_{\sigma}f$ and the Wigner transform $Wf$ (only the moduli squared of $\F f$
and $\F_{\sigma}f$ are plotted).}
\end{figure}

The width $\sigma$ of the Gaussian function $G[a,\Sigma]$ is a
double-edged sword: The smaller it is chosen, the more accurate the
time-frequency description becomes in the $x$-direction, since only values that
are very close to the considered time $x$ contribute to $\F_{\sigma}
f(x,\Cdot)$.
However, the smaller the window, the more  ``difficult'' it becomes to estimate
the frequencies in this small time period and the more ``blurred'' the frequency
decomposition $\F_{\sigma} f(x,\Cdot)$ becomes in $\xi$-direction.
This issue is a manifestation of the so-called uncertainty principle, see the
discussion in \cite[Chapter 2]{grochenig2001foundations}.

The Wigner transform $Wf$ of $f$ provides a way to ``unblurr''
$|\F_{\sigma} f|^2$ at the expense of losing positivity, see Proposition
\ref{prop:husimi} below. It has the proper marginal densities,
\[
\int_{\R^d} Wf(x,\xi)\, \mathrm d\xi\
\ =\  
|f(x)|^2\, ,
\qquad
\int_{\R^d} Wf(x,\xi)\, \mathrm dx
\ =\
|\F f(\xi)|^2\, ,  
\]
but, in general, fails to be non-negative.

\begin{proposition}
\label{prop:husimi}
Let $\displaystyle G_{\sigma}(x,\xi) = \left(2\pi\sigma^2\right)^{-d/2}
\exp\left(-\frac{\|x\|^2+\|\xi\|^2}{2\sigma^2}\right)$
denote a Gaussian in phase space. Then 
\[
Wf \ast G_{1/\sqrt{2}} = |\mathcal \F_{1} f|^2.
\]
\end{proposition}

\begin{proof}
See \cite[(3.10)]{hillery1997distribution}.
\end{proof}














\subsection{Transformations and the Adaptation Function $\mu$}
We are now ready to construct an adaptation function $\mu_f$ that fulfills the
Adaptation Conditions \ref{cond:adaptation}, including condition (iv).
In favor of a better overview, the proofs of Propositions \ref{prop:muFourier},
\ref{prop:muFBI} and \ref{prop:muWigner} will be omitted, since
they are all analogous to the one of Proposition \ref{prop:muWigner2} (the
most complicated one).


Let us start with a \emph{global} version.
A natural way to globally describe the variation of a function $f\in
L^1(\R^d,\R)$ is to consider its Fourier transform, since functions with high
oscillations tend to have high values of $\F f$ away from the origin.
Also, if a function $f\in L^1(\R^d)$ is scaled by some factor $\alpha\neq 0$,
$\tilde f(x) = f(\alpha x)$, the frequencies ``appearing" in the Fourier
transform are scaled by $\alpha^{-1}$:
\begin{equation}
\label{equ:scaleFourier}
\F\tilde f (\xi)
=
(2\pi)^{-d/2} \int_{\R^d} f(\alpha y)\, e^{-iy^\intercal\xi}\,
\mathrm dy
=
\frac{(2\pi)^{-d/2}}{\alpha^d} \int_{\R^d} f(y)\, e^{-iy^\intercal\xi/\alpha}\,
\mathrm dy
=
% \frac{\F f(\xi /\alpha)}{\alpha^d}
\alpha^{-d}\F f(\xi /\alpha)
\, .
\end{equation}
In order to assign a value for the variation to a function $f$, we will
therefore consider the expectation value and covariance defined in the
following proposition:
\begin{proposition}
\label{prop:muFourier}
Let $f\in W^{2,2}(\R^d,\R)\setminus\{0\}$. The expectation value and covariance
matrix of the probability distribution $\P_\rho$ given by the density
\[
\rho = \frac{|\F f|^2}{\|\F f\|_{L^2}^2} = \frac{|\F
f|^2}{\|f\|_{L^2}^2}
\]
(here we used the Plancherel theorem \ref{prop:fourierInverse}) are:
\[
\E_{\rho} = 0
\qquad\text{and}\qquad
\Cov_\rho = \frac{\int_{\R^d} \left(\nabla f\, \nabla
f^{\intercal} - f\, D^2 f\right)(z)\, \mathrm dz}{2\|f\|_{L^2}^2}\, .
\]
\end{proposition}
\begin{proof}
The proof is analogous to the one of Proposition \ref{prop:muWigner2}.
% Since for real-valued functions $f$
% \[
% \F f(-\xi)
% =
% (2\pi)^{-d/2} \int_{\R^d} f(y)\, e^{iy^\intercal\xi}\, \mathrm dy
% =
% (2\pi)^{-d/2} \overline{\int_{\R^d} f(y)\, e^{-iy^\intercal\xi}\, \mathrm dy}
% =
% \overline{\F f(\xi)},
% \]
% the expectation value of $\P_\rho$ vanishes. Using the transformation
% \[
% z_1 = y_1-y_2,\qquad z_2 = y_1+y_2
% \]
% we compute:
% \begin{align*}
% \int_{\R^d} |\F f(\xi)|^2\, \|\xi\|^2\, \mathrm d\xi
% &=
% (2\pi)^{-d}\int_{\R^{3d}} f(y_1)\, f(y_2)\, e^{-i(y_1-y_2)^\intercal\xi}\
% \xi\xi^{\intercal}\, \mathrm dy_1\, \mathrm dy_2\, \mathrm d\xi
% \\
% &=
% \frac{(2\pi)^{-d}}{2^d}\int_{\R^{3d}} \underbrace{
% f\left(\frac{z_2+z_1}{2}\right)\, f\left(\frac{z_2-z_1}{2}\right)}_{=:\,
% F(z_1,z_2)}\, e^{-iz_1^\intercal\xi}\ \xi\xi^\intercal\ \mathrm dz_1\, \mathrm
% dz_2\, \mathrm d\xi
% \\
% &=
% -\frac{(2\pi)^{-d}}{2^d} \int_{\R^{3d}} D_{z_1}^2F(z_1,z_2)\, 
% e^{-iz_1^\intercal\xi}\, \mathrm dz_1\, \mathrm d\xi\, \mathrm dz_2
% \\
% &=
% -\frac{1}{2^d} \int_{\R^d} D_{z_1}^2F(0,z_2)\, 
% \mathrm dz_2
% \\
% &=
% \frac{1}{2}\int_{\R^d} \left(\nabla f\, \nabla f^{\intercal} - f\, D^2
% f\right)(z)\, \mathrm dz.
% \end{align*}
% This proves the formula for the covariance matrix.
\end{proof}


The adaptation function $\mu_f$, which in this global setting is just a constant
adaptation matrix $\mu_f\in\gldr$, can now be assigned the square
root of the covariance matrix $\Cov_\rho$,
\[
\mu_f := \sqrt{\Cov_\rho},
\]
and the Adaptation Conditions \ref{cond:adaptation} can easily be verified (in a
global, $x$-independent sense).

However, we are not interested in a \emph{global}, but in a \emph{local}
adaptation. Therefore, we will study the ``local frequencies'' of $f$ by taking
its windowed Fourier transform $\F_{\sigma} f(x,\xi)$ instead of its Fourier
transform.

Again, let us consider the expectation value and covariance of the corresponding
probability density in $\xi$:
\begin{proposition}
\label{prop:muFBI}
Let $f\in W^{2,2}(\R^d,\R)\setminus\{0\}$. Then, for each $x\in\R^d$, the
expectation value and covariance matrix of the probability distribution $\P_{\rho_x}$ given
by the density
\[
\rho_x = \frac{|\F_\sigma f(x,\Cdot)|^2}{\|\F_\sigma f (x,\Cdot)\|_{L^2}^2}
\]
are:
\[
\E_{\rho_x} = 0
\qquad\text{and}\qquad
\V_{\rho_x} = \frac{\Id}{2\sigma^2} + \frac{\left( \nabla f\nabla f^{\intercal}
- f\, D^2 f\right) \ast G[0,\sigma^2\Id]^2}{2 f^2 \ast
G[0,\sigma^2\Id]^2}(x)\, .
\]
\end{proposition}
\begin{proof}
The proof is analogous to the one of Proposition
\ref{prop:muWigner2}.
% \textcolor{blue}{(In dem Beweis muss $g_{\sigma}$ durch $G[0,\sigma^2\Id]$
% ersetzt werden!)}
% Since for real-valued functions $f$
% \begin{align*}
% \F_\sigma f(x,-\xi)
% &=
% (\pi)^{-d/4} \int_{\R^d} f(y)\, g_\sigma(x-y)\, e^{iy^\intercal\xi}\, \mathrm dy
% \\[0.1cm]
% &=
% (\pi)^{-d/4} \overline{\int_{\R^d} f(y)\, g_\sigma(x-y)\, e^{-iy^\intercal\xi}\,
% \mathrm dy} =
% \overline{\F_\sigma f(x,\xi)},
% \end{align*}
% the expectation value of $\P_{\rho_x}$ vanishes. Using the transformation
% \[
% z_1 = y_1-y_2,\qquad z_2 = y_1+y_2
% \]
% and denoting
% \[
% F_x(z_1,z_2,x) := f\left(\frac{z_2+z_1}{2}\right)\,
% f\left(\frac{z_2-z_1}{2}\right)\, g_\sigma\left(x-\frac{z_2+z_1}{2}\right)\,
% g_\sigma\left(x-\frac{z_2-z_1}{2}\right),
% \]
% we compute
% \begin{align*}
% \int_{\R^d} |\F_{\sigma} f(x,\xi)|^2\, \mathrm d\xi
% &=
% \pi^{-d/2}\int_{\R^{3d}} f(y_1)\, f(y_2)\, g_\sigma(x-y_1)\, g_\sigma(x-y_2)\,
% e^{-i(y_1-y_2)^\intercal\xi}\ \mathrm dy_1\, \mathrm dy_2\, \mathrm d\xi
% \\
% &=
% \frac{\pi^{-d/2}}{2^d}\int_{\R^{3d}} F(z_1,z_2,x)\,
% e^{-iz_1^\intercal\xi}\  \mathrm dz_1\, \mathrm dz_2\, \mathrm d\xi
% \\
% &=
% \pi^{d/2} \int_{\R^d} F(0,z_2,x)\,
% \mathrm dz_2
% \\
% &=
% 2^d\pi^{d/2}\int_{\R^d} f(z)^2 \, g_\sigma(x-z)^2\, \mathrm dz
% \\
% &=
% 2^d\pi^{d/2}\left(f^2\ast g_\sigma^2\right)(x)
% \end{align*}
% and
% \begin{align*}
% &\quad\int_{\R^d} |\F_{\sigma} f(x,\xi)|^2\, \|\xi\|^2\, \mathrm d\xi
% \\
% &=
% \pi^{-d/2} \int_{\R^{3d}} f(y_1)\, f(y_2)\, g_\sigma(x-y_1)\,
% g_\sigma(x-y_2)\, e^{-i(y_1-y_2)^\intercal\xi}\ \|\xi\|^2\, \mathrm dy_1\, \mathrm dy_2\, \mathrm d\xi
% \\
% &=
% \frac{\pi^{-d/2}}{2^d}\int_{\R^{3d}} F(z_1,z_2,x)\, e^{-iz_1^\intercal\xi}\
% \xi^\intercal\xi\ \mathrm dz_1\, \mathrm dz_2\, \mathrm d\xi
% \\
% &=
% -\frac{\pi^{-d/2}}{2^d} \int_{\R^{3d}}D_{z_1}^2F(z_1,z_2,x)\,
% e^{-iz_1^\intercal\xi}\, \mathrm dz_1\, \mathrm d\xi\, \mathrm dz_2
% \\
% &=
% -\pi^{d/2} \int_{\R^d} D_{z_1}^2F(0,z_2,x)\,
% \mathrm dz_2
% \\
% &=
% 2^{d-1}\pi^{d/2}\int_{\R^d} \Big(\sigma^{-2}f(z)^2\Id + \nabla f(z)\nabla
% f(z)^\intercal - f(z)\, D^2f(z)\Big) \, g_\sigma(x-z)^2\, \mathrm dz
% \\
% &=
% 2^{d-1}\pi^{d/2}\Big[\left(\sigma^{-2}f^2\Id + \nabla f\nabla f^{\intercal} -
% f\, D^2 f\right) \ast g_\sigma^2 \Big](x)
% \end{align*}
% Taking the quotient proves the formula for the covariance matrix.
\end{proof}



Again, we can set
\begin{equation}
\label{equ:FBIChoiceMu}
\mu_f(x) := \sqrt{\Cov_{\rho_x}} = \sqrt{\frac{\Id}{2\sigma^2} + \frac{\left( \nabla f\nabla f^{\intercal}
- f\, D^2 f\right) \ast G[0,\sigma^2\Id]^2}{2 f^2 \ast
G[0,\sigma^2\Id]^2}(x)}\ .
\end{equation}
However, while the Adaptation Conditions \ref{cond:adaptation} (i) and (ii) are
fulfilled, the scale invariance (iii) is violated. The reason for this is
that the window of the windowed Fourier transform $\F_\sigma f$ does not scale with the local
variation of $f$, producing the obstructive term $\frac{\Id}{2\sigma^2}$.
A formula analogous to (\ref{equ:scaleFourier}) does not hold for
windowed Fourier transforms.
One might try to adapt the width $\sigma$ of the window locally, but
this would require a priori knowledge of the local variation $\mu_f$ of $f$,
which we are trying to find in the first place.
Another disadvantage of this choice of $\mu_f$ is the difficulty to calculate
the convolutions in the numerator and denominator in practice.

Since the obstructive term is caused by the width of the window, or in other
words, by the blurry way we look at the function, we will ``unblurr'' it by
replacing the term $|\F_\sigma f(x,\xi)|^2$ in the
probability density $\rho_x$ from Proposition \ref{prop:muFBI} with the Wigner
transform $Wf(x,\xi)$. This replacement is motivated by the discussion in
Section \ref{section:PhaseSpace} and by Proposition \ref{prop:husimi} in
particular.

In contrast to the windowed Fourier transform, a formula analogous to
\eqref{equ:scaleFourier} holds for Wigner transforms (again, $\tilde f(x) :=
f(\alpha x)$ for some $\alpha \neq 0$):
\begin{align*}
W\tilde f(x,\xi)
&=
(2\pi)^{-d} \int_{\R^d}\overline{f\left(\alpha x+\frac{\alpha
y}{2}\right)}\, f\left(\alpha x-\frac{\alpha y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy
\\
&=
\frac{(2\pi)^{-d}}{\alpha^d} \int_{\R^d}\overline{f\left(\alpha
x+\frac{y}{2}\right)}\, f\left(\alpha x-\frac{y}{2}\right)\,
e^{iy^\intercal\xi/\alpha}\, \mathrm dy
\\
&=
\alpha^{-d}\, W f(\alpha x,\xi/\alpha).
\end{align*}

We would like to remind the reader that the Wigner transform can attain negative
values and is therefore not a probability density function. However, since we
are going to use the Wigner transform only to get a good guess for the choice of
the adaptation function $\mu_f$, we are going to ignore this detail and just
compute the expectation value and covariance matrix as we did before:
\begin{proposition}
\label{prop:muWigner}
Let $f\in W^{2,2}(\R^d,\R)\setminus\{0\}$. Treating
\[
\rho_x = \frac{Wf(x,\Cdot)}{\int_{\R^d}Wf(x,\xi)\,
\mathrm d\xi} = \frac{Wf(x,\Cdot)}{|f(x)|^2}
\]
as a probability density function for each $x\in\R^d$, the expectation
value and covariance matrix of the probability distribution $\P_{\rho_x}$ are
given by
\[
\E_{\rho_x} = 0
\qquad\text{and}\qquad
\Cov_{\rho_x} = \frac{\nabla f\nabla f^{\intercal} - f\,
D^2 f}{2 f^2}\, (x).
\]
\end{proposition}

\begin{proof}
The proof goes analogously to the one of Proposition \ref{prop:muWigner2}.
% Since the Wigner transform is real-valued, we get for real-valued functions $f$
% \begin{align*}
% W f(x,-\xi)
% &=
% (2\pi)^{-d}\int_{\R^d}f\left(x+\frac{y}{2}\right)\,
% f\left(x-\frac{y}{2}\right)\, e^{-iy^\intercal\xi}\, \mathrm dy
% \\[0.1cm]
% &=
%  (2\pi)^{-d}\overline{\int_{\R^d}f\left(x+\frac{y}{2}\right)\,
% f\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy}
% =
% \overline{W f(x,\xi)}
% =
% W f(x,\xi),
% \end{align*}
% and therefore the expectation value of $\P_{\rho_x}$ vanishes. For the
% covariance matrix we compute:
% \begin{align*}
% \int_{\R^d }W f(x,\xi)\, \xi\xi^{\intercal}\, \mathrm d\xi
% &=
% (2\pi)^{-d} \int_{\R^{2d} } \underbrace{f\left(x+\frac{y}{2}\right)\,
% f\left(x-\frac{y}{2}\right)}_{=:\, F(x,y)}\, e^{iy^\intercal\xi}\,
% \xi\xi^{\intercal}\, \mathrm dy \, \mathrm d\xi
% \\
% &=
% -(2\pi)^{-d} \int_{\R^{3d}} D_y^2F(x,y)\, 
% e^{iy^\intercal\xi}\, \mathrm dy \, \mathrm d\xi
% \\
% &=
% -D_y^2F(x,0)
% \\
% &=
% \frac{1}{2}\left(\nabla f\nabla f^{\intercal} - f\,
% D^2 f\right)(x).
% \end{align*}
% Taking the quotient proves the formula for the covariance matrix.
\end{proof}
\ \\
This time, if we choose 
\begin{equation}
\label{equ:WignerChoiceMu}
\mu_f(x) := \sqrt{\Cov_{\rho_x}} = \sqrt{\frac{\nabla f\nabla f^{\intercal} - f\,
D^2 f}{2 f^2}\, (x)}\, ,
\end{equation}
the Adaptation Conditions \ref{cond:adaptation} are fulfilled. Also, the
cumbersome integrals resulting from convolutions no longer exist, making the application of $\mu_f$
very simple in practice, once the first and second derivatives of $f$ are known.

However, $\Cov_{\rho_x}$ can fail to be positive definite, since the Wigner
transform is not a probability density (it can even become negative definite),
making \eqref{equ:WignerChoiceMu} ill-defined.
In dimension $d=1$, this problem could be approached by choosing 
\begin{equation*}
\mu_f(x) 
=
\sqrt{ \frac{\left| f'(x)^2 - f(x)\, f''(x)\right| + \epsilon_1}{2
f(x)^2 + \epsilon_2}}\ .
\end{equation*}
with small positive numbers
$0<\epsilon_1, \epsilon_2\ll 1$. This solution yields rather satisfactory
results as can be seen in Figure \ref{fig:convolution6und7und8}, but it ``slightly''
violates the Adaptation Conditions (ii)--(iii) and also the
compliance of Adaptation Condition (iv) is unclear,
since we modified the derived adaptation function $\mu_f$.
In higher dimensions one might consider the
LDL-decomposition $M_f=LDL^{\intercal}$ of $M_f := \nabla f\, \nabla
f^{\intercal} - f\, D^2f$ and replace the diagonal of $D$ with its modulus plus
a small positive number $\epsilon_1>0$:
\[
\mu_f(x) 
=
\sqrt{ \frac{L (|D|+\epsilon_1\, \Id)L^{\intercal}}{2
f(x)^2 + \epsilon_2}}\ .
\]
Before considering a more elegant approach to avoid the lack of positive
definiteness, let us state one more result, which suggests a possibility
to calibrate the original width of the smoothing kernel $g$:



\begin{proposition}
\label{prop:gaugeWidth1}
If $f = G[a,\Sigma]$ is a Gaussian density with mean $a\in\R^d$ and covariance
matrix $\Sigma\in\gldr$, then $\mu_f$, as chosen in \eqref{equ:WignerChoiceMu},
is the constant matrix $\mu_f \equiv \sqrt{\frac{1}{2}\Sigma^{-1}}$.
\end{proposition}
\begin{proof}
A simple computation shows:
\begin{align*}
Df(x)
&=
-f(x)(x-a)^{\intercal}\Sigma^{-1}
\\
D^2f(x)
&=
f(x)\left[\Sigma^{-1}(x-a)(x-a)^{\intercal}\Sigma^{-1} - \Sigma^{-1}\right]
\\
\left(\nabla f\, \nabla f^{\intercal} - f\, D^2f\right)(x)
&=
f^2(x)\, \Sigma^{-1}.
\end{align*}
\end{proof}
Therefore, in order to gauge the overall extent of the smoothing process,
Gaussian functions $f$ (or just the standard Gaussian) are well suited for the
calibration of the original width of the smoothing kernel $g$.
\\[0.2cm]
As promised above, we will now follow another approach to overcome the lack of
positive-definiteness of $\Cov_{\rho_x}$. Namely, we will consider $|Wf|^2$
instead of $Wf$, which now does not attain negative values and therefore is a
probability density function, if properly normalized.
Obviously, it inherits the scaling property
$|W\tilde f|^2(x,\xi)=\alpha^{-2d}\, |Wf|^2(\alpha x,\xi/\alpha)$ for
$\tilde f(x) = f(\alpha x)$ ($\alpha \neq 0$).





\begin{proposition}
\label{prop:muWigner2}
Let $f\in W^{2,2}(\R^d,\R)\setminus\{0\}$. Then, for each $x\in\R^d$, the
expectation value and covariance matrix of the probability distribution $\P_{\rho_x}$ given
by the density
\[
\rho_x = \frac{|Wf|^2(x,\Cdot)}{\int_{\R^d}|Wf|^2(x,\xi)\,
\mathrm d\xi}
\]
are:
\[
\E_{\rho_x} = 0
\qquad\text{and}\qquad
\Cov_{\rho_x} = \frac{\left(f^2\right)\ast\left(\nabla f\, \nabla f^{\intercal}
- f\, D^2 f\right)}{4 \left(f^2\right)\ast\left(f^2\right)}\, (2x).
\]
\end{proposition}

\begin{proof}
Since the Wigner transform is real-valued, we get for real-valued functions $f$
\begin{align*}
W f(x,-\xi)
&=
(2\pi)^{-d}\int_{\R^d}f\left(x+\frac{y}{2}\right)\,
f\left(x-\frac{y}{2}\right)\, e^{-iy^\intercal\xi}\, \mathrm dy
\\[0.1cm]
&=
 (2\pi)^{-d}\overline{\int_{\R^d}f\left(x+\frac{y}{2}\right)\,
f\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy}
=
\overline{W f(x,\xi)}
=
W f(x,\xi),
\end{align*}
and therefore the expectation value of $\P_{\rho_x}$ vanishes.
For the covariance matrix, we use the transformation
\[
z_1 = y_1-y_2,\qquad z_2 = y_1+y_2
\]
and the function
\[
F(z_1,z_2) = f\left(x+\frac{z_2 + z_1}{4}\right)f\left(x-\frac{z_2 +
z_1}{4}\right)f\left(x+\frac{z_2 - z_1}{4}\right)f\left(x-\frac{z_2 -
z_1}{4}\right)
\]
to compute:
\begin{align*}
&\int_{\R^d }|W f|^2(x,\xi)\, \mathrm d\xi
\\
&=
(2\pi)^{-2d} \int_{\R^{3d} } f\left(x+\frac{y_1}{2}\right)
f\left(x-\frac{y_1}{2}\right)f\left(x+\frac{y_2}{2}\right)
f\left(x-\frac{y_2}{2}\right) e^{i(y_1-y_2)^\intercal\xi}\,
\mathrm dy_1 \mathrm dy_2 \mathrm d\xi
\\
&=
\frac{(2\pi)^{-2d}}{2^d} \int_{\R^{3d}} F(z_1,z_2)\, 
e^{iz_1^\intercal\xi}\, \mathrm dz_1 \, \mathrm d\xi\, \mathrm dz_2
\\
&=
\frac{(2\pi)^{-d}}{2^d} \int F(0,z_2)\, \mathrm dz_2
\\
&=
\frac{(2\pi)^{-d}}{2^d} \int f^2\left(x+\frac{z_2}{4}\right)\,
f^2\left(x-\frac{z_2}{4}\right)\, \mathrm dz_2
\\
&=
2^d\, (2\pi)^{-d} \int f\left(z\right)^2\,
f\left(2x-z\right)^2\, \mathrm dz
\\
&=
2^d\, (2\pi)^{-d}\, \left(f^2\right)\ast\left(f^2\right) (2x),
\\[0.2cm]
&\int_{\R^d }|W f|^2(x,\xi)\, \xi\xi^{\intercal}\, \mathrm d\xi
\\
&=
(2\pi)^{-2d} \int_{\R^{3d} } f\left(x+\frac{y_1}{2}\right)
f\left(x-\frac{y_1}{2}\right)f\left(x+\frac{y_2}{2}\right)
f\left(x-\frac{y_2}{2}\right) e^{i(y_1-y_2)^\intercal\xi}\, \xi\xi^{\intercal}\, 
\mathrm dy_1 \mathrm dy_2 \mathrm d\xi
\\
&=
(2\pi)^{-2d} \int_{\R^{3d} } f\left(x+y_1/2\right)
f\left(x-\frac{y_1}{2}\right)f\left(x+\frac{y_2}{2}\right)
f\left(x-\frac{y_2}{2}\right) e^{i(y_1-y_2)^\intercal\xi}\, \xi\xi^{\intercal}\, 
\mathrm dy_1 \mathrm dy_2 \mathrm d\xi
\\
&=
\frac{(2\pi)^{-2d}}{2^d} \int_{\R^{3d}} F(z_1,z_2)\, 
e^{iz_1^\intercal\xi}\, \xi\xi^{\intercal}\, \mathrm dz_1 \, \mathrm d\xi\,
\mathrm dz_2
\\
&=
-\frac{(2\pi)^{-d}}{2^d} \int D_{z_1}^2 F(0,z_2)\, \mathrm dz_2
\\
&=
\frac{(2\pi)^{-d}}{2^{d+3}} \int
f^2\left(x+\frac{z_2}{4}\right)
\left[
\nabla f\nabla f^{\intercal} - fD^2f
\right]\left(x-\frac{z_2}{4}\right)
\\
&\hspace{2cm}
+
f^2\left(x-\frac{z_2}{4}\right)
\left[
\nabla f\nabla f^{\intercal} - fD^2f
\right]\left(x+\frac{z_2}{4}\right)
\mathrm dz_2
\\
&=
\frac{(2\pi)^{-d}}{2^{d+3}} \int
f^2(z)
\left[
\nabla f\nabla f^{\intercal} - fD^2f
\right]\left(2x-z\right)
% \\
% &\hspace{2cm}
+
f^2\left(2x-z\right)
\left[
\nabla f\nabla f^{\intercal} - fD^2f
\right]\left(z\right)
\mathrm dz_2
\\
&=
2^{d-2}\, (2\pi)^{-d}\, \left(f^2\right)\ast\left[
\nabla f\nabla f^{\intercal} - fD^2f
\right] (2x).
\end{align*}
Taking the quotient proves the formula for the covariance matrix.
\end{proof}
\ \\
This time, if we choose 
\begin{equation}
\label{equ:finalChoiceMu}
\boxed{
\mu_f(x) := \sqrt{\Cov_{\rho_x}} = \sqrt{\frac{\left(f^2\right)\ast\left(\nabla f\, \nabla f^{\intercal}
- f\, D^2 f\right)}{4 \left(f^2\right)\ast\left(f^2\right)}\, (2x)}\, ,
}
\end{equation}
the Adaptation Conditions \ref{cond:adaptation} are fulfilled:

\begin{proposition}
The choice \ref{equ:finalChoiceMu} for $\mu_f$ fulfills the
Adaptation Conditions \ref{cond:adaptation}
\end{proposition}
\begin{proof}
Condition (i) follows from
\begin{align*}
\left(f(\Cdot -a)\ast g(\Cdot -b)\right)(x)
&=
\int f(y-a)\, g(x-y-b)\, \mathrm dy
=
\int f(y)\, g(x-(a+b)-y)\, \mathrm dy
\\
&=
(f\ast g)(x-(a+b)).
\end{align*}
Condition (ii) is trivial and condition (iii) follows from
\begin{align*}
\left(f(A\cdot\Cdot)\ast g(A\cdot\Cdot)\right)(x)
&=
\int f(Ay)\, g(A(x-y))\, \mathrm dy
=
|\det A|^{-1}\int f(y)\, g(Ax-y)\, \mathrm dy
\\
&=
\frac{(f\ast g)(Ax)}{|\det A|}
\end{align*}
in the following way:
\begin{align*}
\mu_{f(A\cdot\Cdot)}^{\intercal}(x)\, \mu_{f(A\cdot\Cdot)}(x)
&=
\frac{f^2(A\cdot\Cdot)\ast\left[A^{\intercal}\, \nabla f(A\cdot\Cdot)\, \nabla
f^{\intercal}(A\cdot\Cdot)A - A^{\intercal}\, f\,
D^2f(A\cdot\Cdot)\, A\right]}{f^2(A\cdot\Cdot)\ast f^2(A\cdot\Cdot)}\, (2x)
\\
&=
\frac{A^{\intercal}\left[f^2\ast\left(\nabla f\, \nabla f^{\intercal} -
f\, D^2f\right)\right]A}{f^2\ast f^2}\, (2Ax)
\\
&=
A^{\intercal}\, \mu_f^{\intercal}(Ax)\, \mu_f(Ax)\, A\, .
\end{align*}
\end{proof}



\begin{figure}[H]
        \centering
        \begin{subfigure}[b]{\textwidth}
                \centering
                \includegraphics[width=1\textwidth]{images/convolution6}                
                \end{subfigure}%
        \vspace{0.2cm}
        \begin{subfigure}[b]{\textwidth}
                \centering
                \includegraphics[width=1\textwidth]{images/convolution7}
        \end{subfigure}        
        \vspace{0.2cm}
        \begin{subfigure}[b]{\textwidth}
                \centering
                \includegraphics[width=1\textwidth]{images/convolution8}
        \end{subfigure}
        \caption{$\mu_f$ as given by formulas
        \eqref{equ:FBIChoiceMu}, \eqref{equ:WignerChoiceMu},
        \eqref{equ:finalChoiceMu} describes locally the variation of $f$. Choosing it as an adaptation function yields a proper local scaling of $g$ and thereby an adequate smoothing of $f$ everywhere.}
        \label{fig:convolution6und7und8}
\end{figure}

Again, Gaussian densities can be used in order to calibrate the width of the
original smoothing kernel $g$:
\begin{corollary}
If $f$ is a Gaussian density as in \eqref{equ:generalGaussian}, then $\mu_f$, as
chosen in \eqref{equ:finalChoiceMu}, is the constant matrix $\mu_f \equiv
\frac{1}{2}\sqrt{\Sigma^{-1}}$ is a constant matrix.
\end{corollary}
\begin{proof}
The proof goes analogously to the one of Proposition \ref{prop:gaugeWidth1}.
\end{proof}


==> sections/KDE.tex <==
\section{Application: Variable Kernel Density Estimation}

Contributions:
\begin{compactitem}
\item Generalization to matrix valued bandwidths
\item Fixed point iteration
\item TODO: Choice of the constant $\kappa$
\item TODO: Choice of the asymptotic behaviour of $\mtm_n$
\end{compactitem}
\vspace{1cm}
A typical problem in density estimation is to recover a density $\rho\colon\R^d\to\R$ from independent and identically distributed samples $y_1,\dots,y_N\stackrel{\rm iid}{\sim}\rho$ from that density.
A widely used nonparametric technique is kernel density estimation (KDE), which approximates $\rho$ by
\begin{equation}
\label{equ:kde}
\hat{\rho}(x)
=
\frac{1}{N}\sum_{n=1}^{N} K_h\left(x-y_n\right)
=
\frac{1}{Nh}\sum_{n=1}^{N} K\left(h^{-1}(x-y_n)\right),
\end{equation}
where $K\colon \R^d\to\R$ is the so-called kernel, which from now on we will assume to be a probability density function, and $h>0$ the bandwidth.
For $N\to\infty$, the kernel density estimate $\hat{\rho}$ converges to $\rho\ast K_h$, which can be considered a good approximation for small $h$.
%($h$ is usually chosen in dependence of $N$, a common choice is $h\propto N^{-\frac{1}{d+4}}$)

The choice of the bandwidth (for finite $N\in\N$) is a difficult task which until now remains an open problem. Choosing it too small would result in peaked behavior of $\hat{\rho}$, choosing it too large causes oversmoothing.

In order to tackle this trade-off, a lot of effort has been put into the optimal choice of the bandwidth $h$, see TODO REF, where optimality is usually measured by the \emph{mean integrated squared error} (MISE):
\[
h_{\rm opt}
=
\argmin_h \, \MISE (h)
=
\argmin_h \, \E\left[\int (\hat{\rho}(x) - \rho(x))^2\, \mathrm dx\right].
\]
In most cases, $\MISE (h)$ is not computable, since it requires access to the unknown density $\rho$ (it is then often replaced by its asymptotic approximation $\AMISE(h)$).
In special cases, however, in which $\rho$ is known, $\MISE(h)$ and $h_{\rm opt}$ can be computed explicitly. If both $\rho$ and $K$ are the $d$-variate standard Gaussian density, $h_\opt$ is given by
\begin{equation}
\label{equ:hOptGaussian}
h_\opt = \left(\frac{4}{(2d+1)N}\right)^{\frac{1}{d+4}},
\end{equation}
see \cite[Section 4.3.2]{silverman1986density}, which in the univariate case is referred to as Silverman's rule of thumb.
%In the univariate case and for approximately Gaussian densities $\rho$, this results in the so-called Silverman's rule of thumb:
%\[
%h \approx 1.06\, \hat{\sigma}_N\, N^{-\frac{1}{5}},
%\]
%where $\hat{\sigma}_N$ is the standard deviation of the samples $y_1,\dots,y_N$.

While $h_\opt$ is the best choice (as measured by the MISE), it still causes oversmoothing in regions of high point density and can produce peaked behavior of $\hat{\rho}$ in regions where only few points lie.
\emph{Variable kernel density estimation} (or \emph{variable kernel smoothing}) tries to overcome this downside by adapting $h$ \emph{locally}. Roughly speaking there are two possibilities to do so (we adopt the notation of \cite{jones1990variable}, where a graphic illustration of the two estimators can also be found; the indices $V$ and $L$ stand for ``varying'' and ``local''):
\begin{itemize}
\item sample-point estimator, employing a different bandwidth for each data point $y_n$:
\[
\hat{\rho}_V(x)
=
\frac{1}{N}\sum_{n=1}^{N} |\det h(y_n)|^{-1} K\left(h(y_n)^{-1}(x-y_n)\right),
\]
\item balloon estimator, for which the bandwidth varies with the estimation location $x$:
\[
\hat{\rho}_L(x)
=
\frac{1}{N}\sum_{n=1}^{N} |\det h(x)|^{-1} K\left(h(x)^{-1}(x-y_n)\right).
\]
\end{itemize}
Here, we generalize the standard definition to matrix-valued $h\in\mathrm{GL} (d,\R)$, such that the kernel can be stretched and rotated in space. From now on, we will concentrate on sample-point estimators, since they result in probability density functions by construction (in contrast to balloon estimators!) and correspond to adaptive convolutions in the pointwise limit for $N\to\infty$:
\[
\hat{\rho}_V
\xrightarrow{N\to\infty}
%\int |\det h(y)|^{-1} K\left(h(y)^{-1}(\Cdot -y)\right) \mathrm dy
%\ =\ 
\rho\ast_\mu K,
\qquad
\mu := h^{-1}.
\]







\subsection{Scalar bandwidths}
Let us first deal with the case of scalar bandwidths $h>0$ before discussing the matrix-valued case.
Since we prefer peaked kernels in areas of high density and flat kernels in areas of low density,
%In areas of high density many points $y_n$ are lying and hence peaked kernels are preferred.
%In areas of low density, there are only few points $y_n$ and hence flat kernels are preferred.
%Therefore,
a dependence of the form 
%\begin{equation}
%\label{equ:hLaw}
%h_n := h(y_n) \propto \rho(y_n)^{-\beta},\quad \beta >0,
%\end{equation}
\begin{equation}
\label{equ:hLaw}
\mtm_n := h(y_n)^{-1} \propto\, \rho(y_n)^{\beta},\quad \beta >0,
\end{equation}
appears natural.
While \cite{zbMATH03591205} suggest $\beta = 1/d$, which guarantees consistency of the estimator $\hat\rho_V$ under scaling, \cite{zbMATH03800791} argues that $\beta = 1/2$ should be used independent of the dimension.

While \cite{zbMATH03800791} argues that $\beta = 1/2$ should be used independent of the dimension, \cite{zbMATH03591205} suggest $\beta = 1/d$, which guarantees consistency of the estimator $\hat\rho_V$ under scaling --- if $\rho'(x) = \alpha^d\rho(\alpha x)$ and $y_n' = \alpha^{-1}y_n$, $n=1,\dots,N$ are both scaled in space by a factor $\alpha>0$, the estimate is scaled correspondingly:
\begin{equation}
\label{equ:simpleScalingEstimator}
\hat \rho_V'(x) = \alpha^d\, \hat \rho_V(\alpha x).
\end{equation}

Since the unknown density $\rho$ is not accessible, asymptotic approximations of the law \eqref{equ:hLaw} have to be applied by using the distance to the ($k$th) nearest neighbor of $y_n$ (\cite{zbMATH03591205}) or pilot kernel density estimates of $\rho$ with a fixed bandwidth (\cite{abramson1982arbitrariness}).
Surprisingly, the application of a fixed point iteration for the inverse bandwidth $\mtm = (\mtm_n)_{n=1,\dots,N}$ instead of just a pilot estimate has not yet been suggested (to the author's best knowledge).
We propose the iteration
%\begin{equation}
%\label{equ:densityFixedPointIteration}
%\hat \rho_{k+1} = \phi(\hat \rho_k),
%\qquad
%\phi(\hat \rho) := \frac{1}{N}\sum_{n=1}^{N} VORFAKTOR K\left(\frac{\hat \rho(y_n)^\beta}{h_C}(\Cdot - y_n)\right),
%\end{equation}
\begin{equation}
\label{equ:densityFixedPointIteration}
\mtm_n^{(k+1)} =\kappa\, \rho_{\mtm^{(k)}}  (y_n)^{\beta},
\qquad
\rho_\mtm(x) := \frac{1}{N} \sum_{n=1}^{N} \mtm_n\, K\big(\mtm_n(x - y_n)\big),
\end{equation}
where $\kappa>0$ denotes the proportionality constant in \eqref{equ:hLaw}.

\begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{images/myKDEopacityPlot}
\caption{The fixed point iteration \eqref{equ:densityFixedPointIteration} for $N=100$ sample points $y_n\stackrel{\rm iid}{\sim}\rho$ sampled from the true density $\rho$
started with wide and equal bandwidths of the kernels (small $\mtm_n$ for all $n=1,\dots,N$). Here, the constant $\kappa$ was chosen manually.
\textcolor{blue}{Evtl Clipping erwaehnen}
}
\label{fig:densityFixedPointIteration}
\end{figure}


TODO: Convergence of the fixed point iteration unclear. Self-consistency betonen.


==> sections/PhaseSpace.tex <==
\subsection{Phase Space Transformations}
\label{section:PhaseSpace}

In this section, we will discuss three transformations, which allow us to get a
grip on the (local) variation of a function.
All three transformations can be viewed from various perspectives and we will
focus on the time-frequency point of view. In the following, $\mathcal
S(\R^d,\C)$ will denote the Schwartz space of rapidly decreasing functions.

\begin{definition}[Gaussian, Fourier transform, windowed Fourier transform,
Wigner transform]
\ \\
We define
\begin{enumerate}[(i)]
  \item the \emph{Gaussian function} $G[a,\Sigma]\colon \R^d\to\R$ with mean
  $a\in\R^d$ and symmetric and positive definite covariance matrix $\Sigma\in\gldr$,   
  \item the \emph{Fourier transform} $\F: \mathcal S(\R^d,\C)\to \mathcal
  S(\R^d,\C)$,
  \item the \emph{windowed Fourier transform} $\F_{\sigma}:
  \mathcal S(\R^d,\C)\to \mathcal S(\R^d\times \R^d,\C)$ with window width
  $\sigma>0$,
  \item the \emph{Wigner transform} $W: \mathcal S(\R^d,\C)\to \mathcal
  S(\R^d\times\R^d,\R)$ by
\footnote{Usually, the Wigner transform
%$W: \mathcal S(\R^d,\C)\times S(\R^d,\C)\to \mathcal S(\R^d\times\R^d,\C)$
is defined by
$
\displaystyle
W(f,g)(x,\xi) = (2\pi)^{-d}\int_{\R^d}\overline{f\left(x+\frac{y}{2}\right)}\,
g\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy.
$
We will only use its definition on the diagonal, $Wf := W(f,f)$, where it is
real-valued, which can be seen by applying the transformation $y\mapsto -y$ in
the integral.}
\end{enumerate}
\begin{align}
\label{equ:generalGaussian}
G[a,\Sigma](x)
&=
(2\pi)^{-d/2}\, |\det \Sigma|^{-1/2}\,
\exp\left[-\frac{1}{2}(x-a)^{-\intercal}\Sigma^{-1} (x-a)\right],
\\
\mathcal F f (\xi)
&=
(2\pi)^{-d/2} \int_{\R^d} f(y)\, e^{-iy^\intercal\xi}\,
\mathrm dy\, ,
\\
\label{equ:windowedFourier}
\F_{\sigma} f(x,\xi)
&=
\pi^{-d/4} \int_{\R^d}f(y)\, G[0,\sigma\, \Id](x-y)\,
e^{-iy^\intercal\xi}\, \mathrm dy\, ,
\\
Wf(x,\xi)
&=
(2\pi)^{-d}\int_{\R^d}\overline{f\left(x+\frac{y}{2}\right)}\,
f\left(x-\frac{y}{2}\right)\, e^{iy^\intercal\xi}\, \mathrm dy.
\end{align}
\end{definition}





We will restrict ourselves to very few properties of these transforms, further
properties can be found in e.g. \cite{folland1989harmonic}.

\begin{proposition}[Plancherel Theorem and Fourier Inversion Formula]
\label{prop:fourierInverse}
\ \\
The Fourier transform is an isometric isomorphism with inverse
\[
\mathcal F^{-1} g (x) = (2\pi)^{-d/2} \int_{\R^d} g(\xi)\,
e^{-ix^\intercal\xi}\, \mathrm d\xi\, .
\]
\end{proposition}
\begin{proof}
See \cite{folland1989harmonic}.
\end{proof}
The Fourier inversion formula implies for $f\in\mathcal S(\R^d,\C)$
\[
(2\pi)^{-d} \int_{\R^d} \int_{\R^d} f(x)\,
e^{-ix^\intercal\xi}\, \mathrm d\xi\, \mathrm dx
\ =\ 
(2\pi)^{-d/2} \int_{\R^d} \F f(\xi)\,  e^{i0^\intercal\xi}\, \mathrm d\xi\, 
\ =\ 
\F^{-1}\F f(0)
\ =\ 
f(0). 
\]
The technique of using ``$(2\pi)^{-d}\int_{\R^d} e^{-ix^\intercal\xi}\, \mathrm
d\xi$'' as a $\delta$-distribution will be used several times in this section.


From the point of view of time-frequency analysis, the Fourier transform yields a
decomposition of the signal $f$ into its frequencies: it
indicates to which extent which frequency $\xi$ occurs in $f$.
However, one is often interested in the local frequencies of $f$, meaning, which
frequencies of $f$ occur at (or around) a specific time $x$. This can be
analyzed using a windowed Fourier transform, also called Gabor transform, which does not
``see'' the values and frequencies of $f$ far from $x$. Applied to each time
$x$, this defines the mapping \eqref{equ:windowedFourier} on phase space.

\begin{figure}[H]
\centering
\begin{subfigure}[b]{0.098\textwidth}
	\centering	
	\includegraphics[width=4\textwidth,angle = 	90]{images/FBI_Wigner2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.392\textwidth}
	\centering	                
	\includegraphics[width=\textwidth]{images/FBI_Wigner3}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.392\textwidth}
	\centering	                
	\includegraphics[width=\textwidth]{images/FBI_Wigner4}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.098\textwidth}
	\centering	
	\includegraphics[width=0.77\textwidth]{images/FBI_Wigner5}
\end{subfigure}

\vfill
\vspace{0.3cm}

\begin{subfigure}[b]{0.098\textwidth}
	\centering
	\phantom{\includegraphics[width=0.94\textwidth]{images/FBI_Wigner3}}	
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.392\textwidth}
	\centering
	\includegraphics[width=\textwidth]{images/FBI_Wigner1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.392\textwidth}
	\centering
	\includegraphics[width=\textwidth]{images/FBI_Wigner1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.098\textwidth}
	\centering
	\phantom{\includegraphics[width=\textwidth]{images/FBI_Wigner3}}
\end{subfigure}
\caption{Visualisation of how different frequencies of a function $f$ are
represented by the Fourier transform $\F f$, the windowed Fourier transform
$\F_{\sigma}f$ and the Wigner transform $Wf$ (only the moduli squared of $\F f$
and $\F_{\sigma}f$ are plotted).}
\end{figure}

The width $\sigma$ of the Gaussian function $g_{\sigma}$ is a
double-edged sword: The smaller it is chosen, the more accurate the
time-frequency description becomes in $x$-direction, since only values very
close to the considered time $x$ are considered for $\F_{\sigma} f(x,\Cdot)$.
However, the smaller the window, the more  ``difficult'' it becomes to estimate
the frequencies in this small region and the more ``blurred'' the frequency
decomposition $\F_{\sigma} f(x,\Cdot)$ becomes in $\xi$-direction.
This issue is the result of the so-called uncertainty principle, see the
discussion in TODO Gröchenig.


However, the Wigner transform $Wf$ of $f$ provides a way to ``unblurr''
$|\F_{\sigma} f|^2$ at the expense of losing positivity. It has the marginal
densities $|f|^2$ and $|\F f|^2$,
\[
\int_{\R^d} Wf(x,\xi)\, \mathrm d\xi\
\ =\  
|f(x)|^2\, ,
\qquad
\int_{\R^d} Wf(x,\xi)\, \mathrm dx
\ =\
|\F f(\xi)|^2\, ,  
\]
but, in general, fails to be non-negative.

It is, indeed, an unblurred version of the windowed Fourier transform, which is
the statement of the following proposition:
\begin{proposition}
\label{prop:husimi}
Let $\displaystyle G_{\sigma}(x,\xi) = \left(2\pi\sigma^2\right)^{-d/2}
\exp\left(-\frac{\|x\|^2+\|\xi\|^2}{2\sigma^2}\right)$
denote a Gaussian in phase space. Then 
\[
Wf \ast G_{1/\sqrt{2}} = |\mathcal \F_{1} f|^2.
\]
\end{proposition}

\begin{proof}
See \cite[(3.10)]{hillery1997distribution}.
\end{proof}
